Introducing MareNostrum5: A European pre-exascale energy-efficient system designed to serve a broad spectrum of scientific workloads

MareNostrum5 is a pre-exascale supercomputer at the Barcelona Supercomputing Center (BSC), part of the EuroHPC Joint Undertaking. With a peak performance of 314 petaflops, MareNostrum5 features a hybrid architecture comprising Intel Sapphire Rapids CPUs, NVIDIA Hopper GPUs, and DDR5 and high-bandwidth memory (HBM), organized into four partitions optimized for diverse workloads. This document evaluates MareNostrum5 through micro-benchmarks (floating-point performance, memory bandwidth, interconnect throughput), HPC benchmarks (HPL and HPCG), and application studies using Alya, OpenFOAM, and IFS. It highlights MareNostrum5's scalability, efficiency, and energy performance, utilizing the EAR (Energy Aware Runtime) framework to assess power consumption and the effects of direct liquid cooling. Additionally, HBM and DDR5 configurations are compared to examine memory performance trade-offs. Designed to complement standard technical documentation, this study provides insights to guide both new and experienced users in optimizing their workloads and maximizing MareNostrum5's computational capabilities.

==> 810-alya.tex <==
\subsection{Alya}


==> 820-openfoam.tex <==
\subsection{OpenFOAM}


==> 830-ifs.tex <==
\subsection{IFS}
\texttt{
-module module -fPIC -fpe0 \\
-convert big\_endian \\
-assume byterecl -align array64byte \\
-traceback -fpic -qopenmp \\
-qopenmp-threadprivate compat \\
-fp-model precise -fp-speculation=safe \\
-qopt-report=2 -qopt-report-phase=all \\
-fast-transcendentals -ftz \\
-finline-functions -finline-limit=1500 \\
-Winline -assume realloc\_lhs \\
-diag-disable=7713 -diag-disable=11021 \\
-diag-disable=10397 -g -O2 -xCORE-AVX512 \\
-qopt-zmm-usage=high -fimf-use-svml=true
}

